Search for excited fermions and leptoquarks at HERA

Recent results on searches for new particles at the electron-proton collider HERA are reported. Based on roughly 40pb-1 of e^+p data taken in the years 1994-1997, the H1 and ZEUS collaborations have derived new exclusion limits for the direct production of excited fermion states and of leptoquarks in different decay channels, including lepton-flavor violating decays. The results of searches for contact interactions further constrain the parameter space for such particles and their couplings in the high-mass regime, where direct production is kinematically prohibited. Also preliminary analyses of the e^-p data taken in 1998 and 1999 do not find signals of new physics.

==> styles/colors.tex <==
\newcommand{\white}{\color{white}}
\newcommand{\black}{\color{black}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\cyan}{\color{cyan}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\yellow}{\color{yellow}}
\definecolor{darkcyan}{rgb}{0.,.6,.8}
\newcommand{\darkcyan}{\color{darkcyan}}
\definecolor{lightblue}{rgb}{0.8,0.95,1}
\newcommand{\lightblue}{\color{lightblue}}
\definecolor{darkblue}{rgb}{0.,0.,.6}
\newcommand{\darkblue}{\color{darkblue}}
\definecolor{lightgreen}{rgb}{0.8,1.,.95}
\newcommand{\lightgreen}{\color{lightgreen}}
\definecolor{darkgreen}{rgb}{0.,.6,0.1}
\newcommand{\darkgreen}{\color{darkgreen}}
\definecolor{darkred}{rgb}{0.9,0.,.2}
\newcommand{\darkred}{\color{darkred}}
\definecolor{lightgray}{gray}{0.9}
\newcommand{\lightgray}{\color{lightgray}}
\definecolor{darkgray}{gray}{0.2}
\newcommand{\darkgray}{\color{darkgray}}
\definecolor{money}{rgb}{0.4,0.8,0.}
\newcommand{\money}{\color{money}}
\definecolor{purple}{rgb}{0.9,0.0,0.8}
\newcommand{\purple}{\color{purple}}
\definecolor{orange}{rgb}{0.9,0.6,0.2}
\newcommand{\orange}{\color{orange}}
\definecolor{newgr}{rgb}{0.2,0.8,0.2}
\newcommand{\newgr}{\color{newgr}}
\definecolor{newbl}{rgb}{0.3,0.6,0.8}
\newcommand{\newbl}{\color{newbl}}
\definecolor{newor}{rgb}{1.0,0.6,0.}
\newcommand{\newor}{\color{newor}}
\definecolor{lightpink}{rgb}{1.0,0.9,0.95}
\newcommand{\lightpink}{\color{lightpink}}
\definecolor{lightmagenta}{rgb}{1.0,0.95,1.0}
\newcommand{\lightmagenta}{\color{lightmagenta}}
\definecolor{lightcyan}{rgb}{0.9,1.0,1.0}
\newcommand{\lightcyan}{\color{lightcyan}}

